Fully Dynamic Maximal Independent Set with Polylogarithmic Update Time

We present the first algorithm for maintaining a maximal independent set (MIS) of a fully dynamic graph---which undergoes both edge insertions and deletions---in polylogarithmic time. Our algorithm is randomized and, per update, takes $O(\log^2 \Delta \cdot \log^2 n)$ expected time. Furthermore, the algorithm can be adjusted to have $O(\log^2 \Delta \cdot \log^4 n)$ worst-case update-time with high probability. Here, $n$ denotes the number of vertices and $\Delta$ is the maximum degree in the graph. The MIS problem in fully dynamic graphs has attracted significant attention after a breakthrough result of Assadi, Onak, Schieber, and Solomon [STOC'18] who presented an algorithm with $O(m^{3/4})$ update-time (and thus broke the natural $\Omega(m)$ barrier) where $m$ denotes the number of edges in the graph. This result was improved in a series of subsequent papers, though, the update-time remained polynomial. In particular, the fastest algorithm prior to our work had $\widetilde{O}(\min\{\sqrt{n}, m^{1/3}\})$ update-time [Assadi et al. SODA'19]. Our algorithm maintains the lexicographically first MIS over a random order of the vertices. As a result, the same algorithm also maintains a 3-approximation of correlation clustering. We also show that a simpler variant of our algorithm can be used to maintain a random-order lexicographically first maximal matching in the same update-time.

==> greedy.tex <==

\section{Useful Properties of Sequential Greedy Maximal Matching}
\label{app:greedy}

In this section we prove the properties of the sequential greedy maximal matching that we used throughout the paper.

The first property concerns the behavior of greedy matching when it is run on an edge-sampled subgraph of a graph. This property is very similar to some results in \cite{DBLP:conf/icml/AhnCGMW15, DBLP:conf/podc/GhaffariGKMR18,DBLP:journals/corr/Konrad} on greedy algorithms for correlation clustering and maximal independent set.

%To our knowledge, a slightly different variant of this property was first proved for a greedy algorithm for correlation clustering \cite{DBLP:conf/icml/AhnCGMW15} and was adopted to that of the greedy maximal independent set algorithm by \cite{DBLP:conf/podc/GhaffariGKMR18,DBLP:journals/corr/Konrad}.

\begin{lemma}\label{lem:edgesamplegreedy}
Fix a graph $G = (V, E)$, let $\pi$ be a permutation over $E$, and let $p \in (0,1]$ be an arbitrary parameter. We define $G_p = (V, E_p)$ to be the random subgraph of $G$ formed wherein each edge in $E$ appears in $E_p$ independently with probability $p$ and define $M := \greedymatching{G_p, \pi}$. For any vertex $v$ and any parameter $\beta \in (0,1/2)$, we have $\deg_{M}^{\text{res}}(v) \leq \frac{\ln (1/\beta)}{p}$ with probability at least $1 - \beta$. 
\end{lemma}
\begin{proof}
Consider the following equivalent method of generating $M$.  We iterate over the edges in $E$ in the order of $\pi$. Upon visiting an edge $e$, if one of its incident edges belongs to $M$, we call it {\em irrelevant} and discard it. Otherwise, we draw a Bernoulli-$p$ random variable $X_e$; if $X_e = 1$, we call $e$ {\em lucky} and add it to $M$ otherwise we call $e$ \emph{unlucky}.

If $v$ is matched in $M$, then $\deg_M^{\text{res}}(v) = 0$. Otherwise, all of its remaining edges in $G[V \setminus M]$ should have been unlucky. That is, every time we encounter an edge $e$ in this process, it must have been irrelevant or we must have chosen $X_e = 0$. Furthermore, in order to have $\deg_M^{\text{res}}(v) > \tau = \frac{\ln(1/\beta)}{p}$,  there must remain at least $\tau$ edges which are not irrelevant. During this process, the probability that all such edges are marked unlucky is at most $(1-p)^\tau \leq \exp(-\tau p) = \beta$.
\end{proof}

The second useful property of the greedy matching is that modifying a single vertex or edge of $G$ does not change the set of matched vertices too much. Note that that the set of \emph{edges} selected for $M$ can change significantly.

\begin{lemma}\label{lem:lipschitzproperties}
	Fix some graph $G(V,E)$ and let $\rho: E \rightarrow [0,1]$ be an associated list of priorities:
	\begin{enumerate}[itemsep=-0.5ex]
		\item If graph $G'$ is derived by removing a vertex of $G$, then there are at most $2$ vertices whose match-status differs in $\greedymatching{G, \rho}$ and $\greedymatching{G', \rho}$.
		\item If graph $G'$ is derived by removing an edge of $G$, then there are at most $2$ vertices whose match-status differs in $\greedymatching{G, \rho}$ and $\greedymatching{G', \rho}$.
		\item If $\rho'$ is derived by changing a single entry of $\rho$, then there are at most $2$ vertices whose match-status differs in $\greedymatching{G, \rho}$ and $\greedymatching{G, \rho'}$.
	\end{enumerate}
\end{lemma}

\begin{proof}
We start with the proof of the first part. Suppose that $G'$ is obtained by removing some vertex $v$ from $G$. Let $M := \greedymatching{G, \rho}$ and $M' := \greedymatching{G', \rho}$. Furthermore, let $D := M \oplus M'$ denote the symmetric difference of $M$ and $M'$, i.e. the set $(M \setminus M') \cup (M' \setminus M)$. Note that the match-status of a vertex $v$ differs in $M$ and $M'$ if and only if its degree in $D$ is one. Therefore, it suffices to show that there are at most two such vertices in $D$.
		
We first claim that $D$ has at most one connected component (apart from singleton vertices). For sake of contradiction, suppose that $D$ has multiple such connected components; fix one component $C$ that does not contain $v$. Let $e$ be the edge in $C$ with the highest priority. The fact that no higher priority edge that is connected to $e$ is part of $M$ or $M'$ (otherwise $e$ would not be the highest priority edge in $C$) shows that $e$ has to belong to both $M$ and $M'$. By definition of $D$, this means that $e \notin D$ which is a contradiction. Next, observe that since $D$ is composed of the edges of two matchings, its maximum degree is at most 2 and thus its unique component is either a path or a cycle. The latter has no vertex of degree one and the former has two; proving part 1 of Lemma~\ref{lem:lipschitzproperties}.

The proof of the other two parts of Lemma~\ref{lem:lipschitzproperties} follows from a similar argument. If an edge $e$ is removed from $G$ or its entry in $\rho$ is changed, then for the same argument, the symmetric difference $M \oplus M'$ of the two greedy matchings $M$ and $M'$ that are obtained would contain only one connected component which has to contain $e$. Since this component is a cycle or a path, the match-statuses of at most two vertices are different in the two matchings.
\end{proof}

The third property is the most subtle: it can be summarized as stating that the presence of any given edge $e $ appearing in $M$ can be determined from a relatively small number of other edges. To make this more precise, let us consider the following query-based method which we refer to as the ``edge oracle'' $\edgeoracle_{\pi}(e)$ for determining whether an edge $e$ appears in $\greedymatching{G, \pi}$:

\begin{titledtbox}{$\edgeoracle_{\pi}(e)$: A query-process to determine whether  $e \in \greedymatching{G, \pi}$.}
	\begin{algorithmic}
		\State Let $e_1, \ldots, e_d$ be the incident edges to $e$ in $G$ sorted such that $\pi(e_1) < \pi(e_2) < \dots < \pi(e_d)$.
		\For{$i = 1, \ldots, d$}
			\If{$\pi(e_i)  < \pi(e)$}
			\State \textbf{if} $\edgeoracle_{\pi}(e_j) = \yes$ \textbf{then return} \no{}
			\EndIf
		\EndFor
		\State \Return \yes{}
	\end{algorithmic}
\end{titledtbox}
	
It is clear that $e \in \greedymatching{G, \pi}$ if and only if $\edgeoracle_{\pi}(e) = \yes{}$.  For any edge $e \in E$, let us define $A(e)$ to be the number of (recursive) calls to $\edgeoracle_{\pi}$ that are generated by running $\edgeoracle_{\pi}(e)$. Translating a result of  Yoshida \etal{}~\cite{DBLP:conf/stoc/YoshidaYI09} for maximal independent set into our context, gives:
\begin{proposition}[\cite{DBLP:conf/stoc/YoshidaYI09}]
\label{prop:greedmatchquery}
Let $G$ be a graph with $m$ edges and $r$ pairs of intersecting edges. If $\pi$ is drawn u.a.r. from permutations on $m$ elements, then $\E_{\pi} [ \sum_{e \in E} A(e) ] \leq O( m + r )$.
\end{proposition}

\begin{proof}
Let $H$ be the line graph of $G$. Then $H$ has $m$ vertices and $r$ edges, and hence has average degree $2r/m$. Also, $\E_{\pi}[A(e)]$ is the expected query complexity of the maximal independent set of $H$ under a random sequential greedy independent set. The result of Yoshida \etal{}~\cite[Theorem 2.1]{DBLP:conf/stoc/YoshidaYI09} implies the following bound on the average value of $A(e)$ in terms of the average degree of $H$:
$$
\frac{1}{m} \E_{\pi} \Big[ \sum_{e \in L} A(e) \Big] \leq 1 + \frac{2r}{m}.
$$
We obtain the stated result by multiplying through by $m$.
\end{proof}






==> highlevel-orig.tex <==
\section{Our Techniques}\label{sec:highlevel}

\newcommand{\msnote}[1]{{\color{red} Madhu: #1}}
In this section we describe the main ideas behind our fully dynamic MIS algorithm. The ideas behind the maximal matching algorithm are similar though some details are different.

As pointed out earlier, our main contribution is to show that it is actually possible to maintain the lexicographically first MIS (LFMIS), under a random permutation of the vertices, at an expected polylogarithmic cost per update. Both the idea of maintaining the lexicographically first MIS and doing so under a random permutation have been considered in the literature before \cite{Censor-HillelHK16, assadisoda}. But the recent and more efficient algorithms involve a more complicated algorithm. In view of this, the return to the more elementary algorithm and asserting that it helps gain efficiency (as opposed to hurting efficiency) may be counterintuitive. In this section we attempt to explain some of the barriers and how our work overcomes them.

The first hurdle behind maintaining the LFMIS is that it may change a lot under updates. But it is also well-known that this situation changes immediately when one picks a random ordering of the vertices (independent of the update sequence). In particular it is well-known~\cite[Theorem~1]{Censor-HillelHK16} that for a random ordering, the expected alteration to the LFMIS after the insertion or deletion of a single edge is $O(1)$. This already shows that maintaining random order LFMIS is sufficient to get an algorithm with $O(1)$ expected adjustments per update. However, unfortunately, it is not clear how to {\em detect} these changes and maintain the LFMIS efficiently: The natural algorithm to do so would do a breadth-first-search (BFS) from the endpoints of the edge being updated, but even exploring the neighborhood of a single vertex in a graph of degree $\Delta$ might require $\Omega(\Delta)$ time, and this is prohibitively expensive for general graphs in which $\Delta$ can be as large as $\Omega(n)$.\footnote{We note that this is precisely the $\Omega(\Delta)$ barrier mentioned in Section 6 of \cite{Censor-HillelHK16}.}

%(We note that this is a problem only for unbounded degree graphs --- which is what we consider here --- and prior works on MIS in bounded-degree graphs~\cite{???} do implement this natural strategy successfully.) This barrier motivated the search for alternate algorithms in the past, but in this work, we overcome this barrier by some careful analysis and data structures.

Our first idea is to maintain not just the LFMIS, but also the ``eliminator'' of every vertex $v$ in the graph. Briefly, given a ranking $\pi:V \to [0,1]$, the eliminator of a vertex $v$ in a graph $G$ under $\pi$ is its neighbor in $G$ of lowest rank that belongs to the LFMIS. (If $v$ is in the LFMIS, then its eliminator is defined to be itself.) Maintaining the eliminators only seems to complicate our task further: (1) Even if the MIS changes by a little, it is conceivable that the eliminators of many vertices might change a lot. (2) And it is still unclear how to find the set of vertices whose eliminators have changed in $o(\Delta)$ time.

For problem (1) we extend the classical analysis \cite{Censor-HillelHK16}, which showed that the MIS changes only by a little after each update, to show that the eliminators are also extremely robust under updates. We stress that this extension is not simple and requires many new ideas. Furthermore, it is crucial for our analysis that we provide this bound for {\em vertex} updates, not just edge updates. Overall, we get the following guarantee which may be of independent interest:

\restatedesc{Theorem~\ref{thm:vertexA}}{informal statement}{For any arbitrary vertex update, the expected number of vertices whose eliminator changes is $O(\log n)$.}


%... \msnote{Say why this might be challenging if we can find a sentence or two. Or say what is new in the analysis.}

Problem (2) turns out to require carefully designed data structures and this is where the rest of the novelty of this work comes in. For each vertex $v$, we partition its neighborhood (dynamically) in two parts, $N^-(v)$ and $N^+(v)$, that are both stored as binary search trees but are indexed and used very differently. The set $N^-(v)$ includes neighbors of $v$ whose eliminators have smaller rank than the eliminator of $v$. Each vertex $u \in N^-(v)$ is indexed by the rank of its (dynamically changing) eliminator. Moreover, the set $N^+(v)$ includes the rest of neighbors of $v$ and every vertex $u \in N^+(v)$ is indexed by its (static) ID. Our first insight is that vertices whose eliminators have small rank are not likely to change their eliminators under many updates. This, roughly speaking, implies that the cost of reindexing $N^-(v)$ is not too much. Our second insight is that the maximum degree in the graph induced on vertices whose eliminators have high ranks is small. Therefore, set $N^+(v)$ will be typically small and the fact that it is not indexed by the rank of its members' eliminators is not troublesome.


We back up these intuitive statements with formal analyses that show that the eliminators for every vertex $v$, and the neighborhoods $N^-$ and $N^+$ can all be maintained in $\poly\log n$ time (expected, over the choice of the ranking $\pi$). Central to this analysis is Lemma~\ref{lem:edgeA} which actually shows that the expected updates are small even when conditioned on the rank of one of the endpoints of the edge being updated. This conditioned analysis plays a crucial role later when we analyze the number of vertices that we need to explore to update our data structures.

Given the data structures above and the analyses, we get a very clean and efficient algorithm to maintain LFMIS under a random order. The data structures are described formally in Section~\ref{sec:datastructures} and the full algorithm is given in Section~\ref{sec:algalg}. The proofs of Theorem~\ref{thm:vertexA} and Lemma~\ref{lem:updatealg} appear in Section~\ref{sec:analysis} and the final analysis of the update-time is presented in Section~\ref{sec:wrapup}.



\smparagraph{Maximal Matching.} It is well-known that an MM of a graph can be found by first taking its line-graph and then constructing an MIS on it. The challenge is that the line-graph may be much larger than the original graph and thus expensive to construct. However, because of the very specific structure of line-graphs, we can indeed implement almost the same algorithm for MM without going through an explicit construction of the line-graph. In what follows, we highlight the main differences between our MIS algorithm and its MM implementation.

The first difference is that for LFMM, the random ranking $\pi$ has to be drawn on the edges instead of the vertices and thus we cannot fix $\pi$ in the pre-processing step. However, this is easy to handle: We draw the rank $\pi(e) \in [0, 1]$ of any edge $e$ randomly upon its arrival.

The second difference is where the specific structure of line-graphs helps significantly. The set of edges whose MM-statuses change as a result of an edge update form a path. In fact, this holds true for any arbitrary ranking $\pi$ over the edges. This is in sharp contrast with MIS, where the propagations may branch (consider a star and assume that the center leaves the MIS). It is well-known that the depth of such alterations are w.h.p. $O(\log n)$ \cite{DBLP:conf/spaa/BlellochFS12,DBLP:conf/soda/FischerN18} if $\pi$ is a random ranking. Therefore, the analogous of Theorem~\ref{thm:vertexA} for MM is significantly easier to prove. It also simplifies the algorithm we use to  detect the changes to MM (compared to MIS).

The third difference is simple but plays a crucial role in adapting the MIS algorithm to MM. Instead of storing the adjacency lists on the edges, which is the natural idea if one constructs the line-graph explicitly, we can simply store them on the vertices. Then, any edge $e$ can access its adjacency lists by looking at those of its two end-points. In fact, it turns out that for MM, we do not need to partition the adjacency lists into $N^+$ and $N^-$ and we can afford to index all the neighboring edges of each vertex by their eliminators' ranks.

In Section~\ref{sec:MM}, we turn all these intuitions into a concrete algorithm that maintains an LFMM of a fully-dynamic graph in $\polylog n$ expected and worst-case update-time.


\iffalse{
Intuition behind the algorithm:

\begin{enumerate}
	\item trivial $O(m)$ approach
	\item chain of changes, can be multiple hops away
	\item we already know very few MIS-status changes occur. the problem is how to detect them.
	\item  Explain an $O(\Delta)$ time algorithm --- but we want better.
	\item Note that it is tricky to determine which neighbor has to join the MIS (figure required). To break $\Delta$, we should not look at all of its neighbors.
	\item Mention the pruning effect of LFMIS. 
	\item Take the lower rank vertex $a$ of $e$. The MIS remains unchanged on the set of vertices with rank smaller than $a$. Therefore, all the changes occur on the remaining graph after processing $[0, \pi(a)]$. The maximum degree on this graph is $\widetilde{O}(\pi(a)^{-1})$, which, in expectation, is $\widetilde{O}(1)$.
	\item But how do we detect which vertices belong to this sparser graph? We need some data structures for this.
	\item For each vertex $v$, we maintain the rank of its eliminator $k(v)$. Now if we maintain $N(v)$ indexed by $k(u)$ we can quickly determine those that survive.
	\item Unfortunately, $N(v)$ is expensive to maintain. Even if $k(v)$ of a single vertex $v$ is changed, we need to update its position in $N(u)$ of each of its neighbors and again hit the $\Omega(\Delta)$ barrier.
	\item To resolve this issue, for each vertex $v$, we maintain two adjacency lists $N^+(v)$ and $N^-(v)$.
	\item Now, observe that instead of MIS, we are maintaining the vertices' eliminators. Let us use $A$ to denote the number of vertices whose eliminators change. We can update all data structures in $\widetilde{O}(A \cdot \pi(a)^{-1})$.
\end{enumerate}

Now, the analysis:

\begin{enumerate}
	\item It is not hard to bound both $\E[A]$ and $\E[\pi(a)^{-1}]$ by $\widetilde{O}(1)$. However, note this is not sufficient to prove $\E[A \cdot \pi(a)^{-1}]$ is small since the two random variables are correlated.
	\item For this, we need to bound $\E[A]$ when we condition on $\pi(a)^{-1}$. For instance, suppose that $\pi(a)$ is very small, say $\Delta^{-1}$. We should still be able to prove $\E[A]$ is small.
	\item To do this, instead of an edge update, we consider the effect of vertex updates. And prove that $\E[A]$ is as small as $O(\log n)$ even when a vertex is removed from the graph.
	\item To do this, we map permutations to each other, etc.
\end{enumerate}

}\fi  
